Graph Representational Learning: When Does More Expressivity Hurt Generalization?

Graph Neural Networks (GNNs) are powerful tools for learning on structured data, yet the relationship between their expressivity and predictive performance remains unclear. We introduce a family of premetrics that capture different degrees of structural similarity between graphs and relate these similarities to generalization, and consequently, the performance of expressive GNNs. By considering a setting where graph labels are correlated with structural features, we derive generalization bounds that depend on the distance between training and test graphs, model complexity, and training set size. These bounds reveal that more expressive GNNs may generalize worse unless their increased complexity is balanced by a sufficiently large training set or reduced distance between training and test graphs. Our findings relate expressivity and generalization, offering theoretical insights supported by empirical results.

==> data/Proteins_TMD_1layer.tex <==
Distance,CumulativeAccuracy
2.0,1.0
2.0,1.0
2.0,0.6666666666666666
2.0,0.5
2.0,0.6
2.0,0.6666666666666666
2.0,0.7142857142857143
2.0,0.75
2.0,0.6666666666666666
2.0,0.7
2.0,0.7272727272727273
2.0,0.75
2.0,0.7692307692307693
2.0,0.7857142857142857
2.0,0.8
2.0,0.8125
2.0,0.8235294117647058
2.0,0.8333333333333334
2.0,0.7894736842105263
2.0,0.8
3.414213538169861,0.8095238095238095
3.414213538169861,0.8181818181818182
3.414213538169861,0.782608695652174
3.414213538169861,0.75
3.414213538169861,0.72
3.414213538169861,0.7307692307692307
3.414213538169861,0.7407407407407407
3.414213538169861,0.75
3.414213538169861,0.7586206896551724
3.414213538169861,0.7666666666666667
3.414213538169861,0.7741935483870968
3.414213538169861,0.78125
3.414213538169861,0.7878787878787878
3.414213538169861,0.7941176470588235
3.414213538169861,0.8
3.414213538169861,0.7777777777777778
3.414213538169861,0.7567567567567568
3.414213538169861,0.7631578947368421
3.414213538169861,0.7692307692307693
3.414213538169861,0.775
4.0,0.7804878048780488
4.0,0.7619047619047619
4.0,0.7674418604651163
4.0,0.75
4.0,0.7555555555555555
4.0,0.7391304347826086
4.0,0.723404255319149
4.0,0.7291666666666666
4.0,0.7346938775510204
4.0,0.74
5.414213538169861,0.7450980392156863
5.414213538169861,0.75
5.414213538169861,0.7547169811320755
5.414213538169861,0.7592592592592593
5.414213538169861,0.7636363636363637
5.414213538169861,0.7678571428571429
5.414213538169861,0.7719298245614035
5.414213538169861,0.7586206896551724
5.414213538169861,0.7457627118644068
5.414213538169861,0.7333333333333333
5.414213538169861,0.7377049180327869
5.414213538169861,0.7419354838709677
5.414213538169861,0.746031746031746
5.414213538169861,0.75
5.414213538169861,0.7538461538461538
5.414213538169861,0.7575757575757576
5.414213538169861,0.7611940298507462
5.414213538169861,0.75
5.414213538169861,0.7391304347826086
5.414213538169861,0.7428571428571429
6.0,0.7464788732394366
6.0,0.7361111111111112
6.0,0.7397260273972602
6.0,0.7432432432432432
6.0,0.7333333333333333
6.0,0.7368421052631579
6.0,0.7402597402597403
6.0,0.7435897435897436
6.0,0.7468354430379747
6.0,0.75
6.2426406145095825,0.7530864197530864
6.2426406145095825,0.7560975609756098
6.2426406145095825,0.7590361445783133
6.2426406145095825,0.75
6.2426406145095825,0.7529411764705882
6.2426406145095825,0.7441860465116279
6.2426406145095825,0.7471264367816092
6.2426406145095825,0.75
6.2426406145095825,0.7415730337078652
6.2426406145095825,0.7333333333333333
6.2426406145095825,0.7362637362637363
6.2426406145095825,0.7391304347826086
6.2426406145095825,0.7419354838709677
6.2426406145095825,0.7446808510638298
6.2426406145095825,0.7473684210526316
6.2426406145095825,0.75
6.2426406145095825,0.7422680412371134
6.2426406145095825,0.7448979591836735
6.2426406145095825,0.7474747474747475
6.2426406145095825,0.75
6.2426406145095825,0.7524752475247525
6.2426406145095825,0.7549019607843137
6.2426406145095825,0.7572815533980582
6.2426406145095825,0.75
6.2426406145095825,0.7523809523809524
6.2426406145095825,0.7452830188679245
6.2426406145095825,0.7476635514018691
6.2426406145095825,0.75
6.2426406145095825,0.7522935779816514
6.2426406145095825,0.7545454545454545
6.414213538169861,0.7567567567567568
6.414213538169861,0.7589285714285714
6.414213538169861,0.7522123893805309
6.414213538169861,0.7543859649122807
6.414213538169861,0.7565217391304347
6.414213538169861,0.7586206896551724
6.414213538169861,0.7606837606837606
6.414213538169861,0.7542372881355932
6.414213538169861,0.7563025210084033
6.414213538169861,0.7583333333333333
7.0,0.7520661157024794
7.0,0.7540983606557377
7.0,0.7479674796747967
7.0,0.75
7.0,0.744
7.0,0.746031746031746
7.0,0.7480314960629921
7.0,0.75
7.0,0.751937984496124
7.0,0.7461538461538462
7.656854152679443,0.7480916030534351
7.656854152679443,0.75
7.656854152679443,0.7443609022556391
7.656854152679443,0.746268656716418
7.656854152679443,0.7407407407407407
7.656854152679443,0.7426470588235294
7.656854152679443,0.7372262773722628
7.656854152679443,0.7318840579710145
7.656854152679443,0.7338129496402878
7.656854152679443,0.7357142857142858
7.656854152679443,0.7375886524822695
7.656854152679443,0.7394366197183099
7.656854152679443,0.7412587412587412
7.656854152679443,0.7361111111111112
7.656854152679443,0.7379310344827587
7.656854152679443,0.7397260273972602
7.656854152679443,0.7414965986394558
7.656854152679443,0.7432432432432432
7.656854152679443,0.7449664429530202
7.656854152679443,0.74
8.242640614509583,0.7417218543046358
8.242640614509583,0.743421052631579
8.242640614509583,0.7450980392156863
8.242640614509583,0.7467532467532467
8.242640614509583,0.7419354838709677
8.242640614509583,0.7371794871794872
8.242640614509583,0.7388535031847133
8.242640614509583,0.740506329113924
8.242640614509583,0.7358490566037735
8.242640614509583,0.7375
8.828427076339722,0.7391304347826086
8.828427076339722,0.7407407407407407
8.828427076339722,0.7361963190184049
8.828427076339722,0.7378048780487805
8.828427076339722,0.7393939393939394
8.828427076339722,0.7349397590361446
8.828427076339722,0.7365269461077845
8.828427076339722,0.7321428571428571
8.828427076339722,0.727810650887574
8.828427076339722,0.7294117647058823
8.828427076339722,0.7251461988304093
8.828427076339722,0.7267441860465116
8.828427076339722,0.7283236994219653
8.828427076339722,0.7298850574712644
8.828427076339722,0.7314285714285714
8.828427076339722,0.7329545454545454
8.828427076339722,0.7344632768361582
8.828427076339722,0.7359550561797753
8.828427076339722,0.7374301675977654
8.828427076339722,0.7388888888888889
9.41421353816986,0.7403314917127072
9.41421353816986,0.7362637362637363
9.41421353816986,0.7377049180327869
9.41421353816986,0.7336956521739131
9.41421353816986,0.7297297297297297
9.41421353816986,0.7311827956989247
9.41421353816986,0.732620320855615
9.41421353816986,0.7340425531914894
9.41421353816986,0.7354497354497355
9.41421353816986,0.7315789473684211
9.41421353816986,0.7277486910994765
9.41421353816986,0.7291666666666666
9.41421353816986,0.7305699481865285
9.41421353816986,0.7319587628865979
9.41421353816986,0.7333333333333333
9.41421353816986,0.7346938775510204
9.41421353816986,0.7360406091370558
9.41421353816986,0.7373737373737373
9.41421353816986,0.7386934673366834
9.41421353816986,0.74
9.656854152679443,0.7412935323383084
9.656854152679443,0.7425742574257426
9.656854152679443,0.7438423645320197
9.656854152679443,0.7450980392156863
9.656854152679443,0.7463414634146341
9.656854152679443,0.7475728155339806
9.656854152679443,0.748792270531401
9.656854152679443,0.7451923076923077
9.656854152679443,0.7464114832535885
9.656854152679443,0.7428571428571429
10.828427076339722,0.7440758293838863
10.828427076339722,0.7452830188679245
10.828427076339722,0.7417840375586855
10.828427076339722,0.7429906542056075
10.828427076339722,0.7441860465116279
10.828427076339722,0.7453703703703703
10.828427076339722,0.7419354838709677
10.828427076339722,0.7431192660550459
10.828427076339722,0.7397260273972602
10.828427076339722,0.740909090909091
11.0,0.7420814479638009
11.0,0.7432432432432432
11.0,0.7443946188340808
11.0,0.7455357142857143
11.0,0.7466666666666667
11.0,0.7433628318584071
11.0,0.7444933920704846
11.0,0.7456140350877193
11.0,0.7467248908296943
11.0,0.7478260869565218
11.656854152679443,0.7489177489177489
11.656854152679443,0.7456896551724138
11.656854152679443,0.7467811158798283
11.656854152679443,0.7478632478632479
11.656854152679443,0.7489361702127659
11.656854152679443,0.75
11.656854152679443,0.7510548523206751
11.656854152679443,0.7521008403361344
11.656854152679443,0.7489539748953975
11.656854152679443,0.75
11.656854152679443,0.7510373443983402
11.656854152679443,0.7520661157024794
11.656854152679443,0.7530864197530864
11.656854152679443,0.75
11.656854152679443,0.7510204081632653
11.656854152679443,0.7520325203252033
11.656854152679443,0.7489878542510121
11.656854152679443,0.7459677419354839
11.656854152679443,0.7429718875502008
11.656854152679443,0.744
12.0,0.7450199203187251
12.0,0.746031746031746
12.0,0.7470355731225297
12.0,0.7440944881889764
12.0,0.7411764705882353
12.0,0.7421875
12.0,0.7431906614785992
12.0,0.7441860465116279
12.0,0.7413127413127413
12.0,0.7423076923076923
12.41421353816986,0.7432950191570882
12.41421353816986,0.7442748091603053
12.41421353816986,0.7452471482889734
12.41421353816986,0.7462121212121212
12.41421353816986,0.7471698113207547
12.41421353816986,0.7481203007518797
12.41421353816986,0.7490636704119851
12.41421353816986,0.75
12.41421353816986,0.7472118959107806
12.41421353816986,0.7444444444444445
12.485281229019165,0.7453874538745388
12.485281229019165,0.7463235294117647
12.485281229019165,0.7472527472527473
12.485281229019165,0.7445255474452555
12.485281229019165,0.7454545454545455
12.485281229019165,0.7463768115942029
12.485281229019165,0.7436823104693141
12.485281229019165,0.7410071942446043
12.485281229019165,0.7419354838709677
12.485281229019165,0.7428571428571429
13.071067690849304,0.7437722419928826
13.071067690849304,0.7446808510638298
13.071067690849304,0.7420494699646644
13.071067690849304,0.7429577464788732
13.071067690849304,0.743859649122807
13.071067690849304,0.7447552447552448
13.071067690849304,0.7456445993031359
13.071067690849304,0.7430555555555556
13.071067690849304,0.740484429065744
13.071067690849304,0.7413793103448276
13.899494767189026,0.7422680412371134
13.899494767189026,0.7431506849315068
13.899494767189026,0.7440273037542662
13.899494767189026,0.7448979591836735
13.899494767189026,0.7423728813559322
13.899494767189026,0.7432432432432432
13.899494767189026,0.7441077441077442
13.899494767189026,0.7449664429530202
13.899494767189026,0.7424749163879598
13.899494767189026,0.7433333333333333
14.242640614509583,0.7441860465116279
14.242640614509583,0.7417218543046358
14.242640614509583,0.7425742574257426
14.242640614509583,0.743421052631579
14.242640614509583,0.740983606557377
14.242640614509583,0.7418300653594772
14.242640614509583,0.742671009771987
14.242640614509583,0.7435064935064936
14.242640614509583,0.7443365695792881
14.242640614509583,0.7419354838709677
14.485281229019165,0.7427652733118971
14.485281229019165,0.7435897435897436
14.485281229019165,0.744408945686901
14.485281229019165,0.7420382165605095
14.485281229019165,0.7428571428571429
14.485281229019165,0.7436708860759493
14.485281229019165,0.7444794952681388
14.485281229019165,0.7452830188679245
14.485281229019165,0.7460815047021944
14.485281229019165,0.746875
14.485281229019165,0.7476635514018691
14.485281229019165,0.7484472049689441
14.485281229019165,0.7461300309597523
14.485281229019165,0.7469135802469136
14.485281229019165,0.7476923076923077
14.485281229019165,0.745398773006135
14.485281229019165,0.746177370030581
14.485281229019165,0.7469512195121951
14.485281229019165,0.7477203647416414
14.485281229019165,0.7484848484848485
14.656854152679443,0.7462235649546828
14.656854152679443,0.7469879518072289
14.656854152679443,0.7477477477477478
14.656854152679443,0.7455089820359282
14.656854152679443,0.746268656716418
14.656854152679443,0.7470238095238095
14.656854152679443,0.7477744807121661
14.656854152679443,0.7485207100591716
14.656854152679443,0.7463126843657817
14.656854152679443,0.7470588235294118
14.828427076339722,0.7478005865102639
14.828427076339722,0.7456140350877193
14.828427076339722,0.7463556851311953
14.828427076339722,0.747093023255814
14.828427076339722,0.7478260869565218
14.828427076339722,0.7456647398843931
14.828427076339722,0.7463976945244957
14.828427076339722,0.7442528735632183
14.828427076339722,0.7449856733524355
14.828427076339722,0.7428571428571429
15.071067690849304,0.7407407407407407
15.071067690849304,0.7386363636363636
15.071067690849304,0.7393767705382436
15.071067690849304,0.7401129943502824
15.071067690849304,0.7408450704225352
15.071067690849304,0.7415730337078652
15.071067690849304,0.7394957983193278
15.071067690849304,0.7374301675977654
15.071067690849304,0.7381615598885793
15.071067690849304,0.7388888888888889
16.14213538169861,0.739612188365651
16.14213538169861,0.7403314917127072
16.14213538169861,0.7410468319559229
16.14213538169861,0.7417582417582418
16.14213538169861,0.7424657534246575
16.14213538169861,0.7404371584699454
16.14213538169861,0.7411444141689373
16.14213538169861,0.7418478260869565
16.14213538169861,0.7398373983739838
16.14213538169861,0.7405405405405405
16.656854152679443,0.7412398921832885
16.656854152679443,0.7419354838709677
16.656854152679443,0.7426273458445041
16.656854152679443,0.7433155080213903
16.656854152679443,0.744
16.656854152679443,0.7420212765957447
16.656854152679443,0.7427055702917772
16.656854152679443,0.7407407407407407
16.656854152679443,0.7387862796833773
16.656854152679443,0.7394736842105263
16.656854152679443,0.7401574803149606
16.656854152679443,0.7408376963350786
16.656854152679443,0.7389033942558747
16.656854152679443,0.7395833333333334
16.656854152679443,0.7376623376623377
16.656854152679443,0.7357512953367875
16.656854152679443,0.7364341085271318
16.656854152679443,0.7371134020618557
16.656854152679443,0.7352185089974294
16.656854152679443,0.735897435897436
16.97056245803833,0.7365728900255755
16.97056245803833,0.7346938775510204
16.97056245803833,0.7353689567430025
16.97056245803833,0.7360406091370558
16.97056245803833,0.7341772151898734
16.97056245803833,0.7348484848484849
16.97056245803833,0.7329974811083123
16.97056245803833,0.7336683417085427
16.97056245803833,0.7343358395989975
16.97056245803833,0.735
17.0,0.7331670822942643
17.0,0.7338308457711443
17.0,0.7320099255583127
17.0,0.7326732673267327
17.0,0.7333333333333333
17.0,0.7339901477832512
17.0,0.7346437346437347
17.0,0.7352941176470589
17.0,0.7334963325183375
17.0,0.7317073170731707
18.071067690849304,0.732360097323601
18.071067690849304,0.7305825242718447
18.071067690849304,0.7312348668280871
18.071067690849304,0.7318840579710145
18.071067690849304,0.7325301204819277
18.071067690849304,0.7331730769230769
18.071067690849304,0.7314148681055156
18.071067690849304,0.7320574162679426
18.071067690849304,0.7326968973747017
18.071067690849304,0.7333333333333333
18.071067690849304,0.7339667458432304
18.071067690849304,0.7322274881516587
18.071067690849304,0.7328605200945626
18.071067690849304,0.7334905660377359
18.071067690849304,0.731764705882353
18.071067690849304,0.7323943661971831
18.071067690849304,0.7330210772833724
18.071067690849304,0.7313084112149533
18.071067690849304,0.7319347319347319
18.071067690849304,0.7325581395348837
18.242640614509583,0.7331786542923434
18.242640614509583,0.7337962962962963
18.242640614509583,0.7344110854503464
18.242640614509583,0.7327188940092166
18.242640614509583,0.7333333333333333
18.242640614509583,0.7339449541284404
18.242640614509583,0.7345537757437071
18.242640614509583,0.7351598173515982
18.242640614509583,0.7357630979498861
18.242640614509583,0.7340909090909091
19.071067690849304,0.7324263038548753
19.071067690849304,0.7330316742081447
19.071067690849304,0.7313769751693002
19.071067690849304,0.7319819819819819
19.071067690849304,0.7325842696629213
19.071067690849304,0.7331838565022422
19.071067690849304,0.7337807606263982
19.071067690849304,0.7321428571428571
19.071067690849304,0.732739420935412
19.071067690849304,0.7333333333333333
19.485281229019165,0.7317073170731707
19.485281229019165,0.7323008849557522
19.485281229019165,0.7328918322295805
19.485281229019165,0.7334801762114538
19.485281229019165,0.734065934065934
19.485281229019165,0.7346491228070176
19.485281229019165,0.7330415754923414
19.485281229019165,0.7336244541484717
19.485281229019165,0.7342047930283224
19.485281229019165,0.7347826086956522
19.656854152679443,0.735357917570499
19.656854152679443,0.7359307359307359
19.656854152679443,0.7365010799136069
19.656854152679443,0.7370689655172413
19.656854152679443,0.7376344086021506
19.656854152679443,0.7360515021459227
19.656854152679443,0.7366167023554604
19.656854152679443,0.7371794871794872
19.656854152679443,0.7377398720682303
19.656854152679443,0.7361702127659574
19.82842707633972,0.7367303609341825
19.82842707633972,0.7372881355932204
19.82842707633972,0.7378435517970402
19.82842707633972,0.7383966244725738
19.82842707633972,0.7389473684210527
19.82842707633972,0.7394957983193278
19.82842707633972,0.7379454926624738
19.82842707633972,0.7384937238493724
19.82842707633972,0.7390396659707724
19.82842707633972,0.7395833333333334
20.071067690849304,0.738045738045738
20.071067690849304,0.7385892116182573
20.071067690849304,0.7370600414078675
20.071067690849304,0.7355371900826446
20.071067690849304,0.734020618556701
20.071067690849304,0.7345679012345679
20.071067690849304,0.7351129363449692
20.071067690849304,0.735655737704918
20.071067690849304,0.7361963190184049
20.071067690849304,0.736734693877551
20.14213538169861,0.7372708757637475
20.14213538169861,0.7378048780487805
20.14213538169861,0.7363083164300203
20.14213538169861,0.7348178137651822
20.14213538169861,0.7333333333333333
20.14213538169861,0.7338709677419355
20.14213538169861,0.7344064386317908
20.14213538169861,0.7349397590361446
20.14213538169861,0.7354709418837675
20.14213538169861,0.736
20.656854152679443,0.7365269461077845
20.656854152679443,0.7370517928286853
20.656854152679443,0.7375745526838966
20.656854152679443,0.7380952380952381
20.656854152679443,0.7366336633663366
20.656854152679443,0.7371541501976284
20.656854152679443,0.73767258382643
20.656854152679443,0.7381889763779528
20.656854152679443,0.7387033398821218
20.656854152679443,0.7392156862745098
21.0,0.7397260273972602
21.0,0.73828125
21.0,0.7387914230019493
21.0,0.7373540856031129
21.0,0.7359223300970874
21.0,0.7364341085271318
21.0,0.7369439071566731
21.0,0.7374517374517374
21.0,0.7379576107899807
21.0,0.7384615384615385
21.242640614509583,0.7389635316698656
21.242640614509583,0.7394636015325671
21.242640614509583,0.7380497131931166
21.242640614509583,0.7385496183206107
21.242640614509583,0.7390476190476191
21.242640614509583,0.7395437262357415
21.242640614509583,0.7381404174573055
21.242640614509583,0.7386363636363636
21.242640614509583,0.7372400756143668
21.242640614509583,0.7377358490566037
21.485281229019165,0.7382297551789078
21.485281229019165,0.7387218045112782
21.485281229019165,0.7373358348968105
21.485281229019165,0.7378277153558053
21.485281229019165,0.7383177570093458
21.485281229019165,0.7388059701492538
21.485281229019165,0.7374301675977654
21.485281229019165,0.7379182156133829
21.485281229019165,0.738404452690167
21.485281229019165,0.737037037037037
21.82842707633972,0.7375231053604436
21.82842707633972,0.7380073800738007
21.82842707633972,0.7384898710865562
21.82842707633972,0.7371323529411765
21.82842707633972,0.7376146788990826
21.82842707633972,0.7380952380952381
21.82842707633972,0.7385740402193784
21.82842707633972,0.7372262773722628
21.82842707633972,0.7377049180327869
21.82842707633972,0.7381818181818182
21.899494767189026,0.7386569872958257
21.899494767189026,0.7391304347826086
21.899494767189026,0.7377938517179023
21.899494767189026,0.7364620938628159
21.899494767189026,0.736936936936937
21.899494767189026,0.737410071942446
21.899494767189026,0.7360861759425493
21.899494767189026,0.7365591397849462
21.899494767189026,0.7370304114490162
21.899494767189026,0.7375
22.82842707633972,0.7379679144385026
22.82842707633972,0.7384341637010676
22.82842707633972,0.738898756660746
22.82842707633972,0.7375886524822695
22.82842707633972,0.7380530973451327
22.82842707633972,0.7385159010600707
22.82842707633972,0.7389770723104057
22.82842707633972,0.7394366197183099
22.82842707633972,0.7381370826010545
22.82842707633972,0.7385964912280701
22.899494767189026,0.7390542907180385
22.899494767189026,0.7395104895104895
22.899494767189026,0.7382198952879581
22.899494767189026,0.7386759581881533
22.899494767189026,0.7391304347826086
22.899494767189026,0.7395833333333334
22.899494767189026,0.7400346620450606
22.899494767189026,0.740484429065744
22.899494767189026,0.7392055267702936
22.899494767189026,0.7379310344827587
22.899494767189026,0.7366609294320138
22.899494767189026,0.7371134020618557
22.899494767189026,0.7375643224699828
22.899494767189026,0.738013698630137
22.899494767189026,0.7384615384615385
22.899494767189026,0.7389078498293515
22.899494767189026,0.7393526405451448
22.899494767189026,0.7380952380952381
22.899494767189026,0.7385398981324278
22.899494767189026,0.7389830508474576
23.14213538169861,0.739424703891709
23.14213538169861,0.7381756756756757
23.14213538169861,0.7386172006745363
23.14213538169861,0.7390572390572391
23.14213538169861,0.7394957983193278
23.14213538169861,0.7399328859060402
23.14213538169861,0.7386934673366834
23.14213538169861,0.7391304347826086
23.14213538169861,0.7395659432387313
23.14213538169861,0.74
23.313708305358887,0.7387687188019967
23.313708305358887,0.739202657807309
23.313708305358887,0.7396351575456053
23.313708305358887,0.7400662251655629
23.313708305358887,0.740495867768595
23.313708305358887,0.740924092409241
23.313708305358887,0.7413509060955519
23.313708305358887,0.7417763157894737
23.313708305358887,0.7422003284072249
23.313708305358887,0.7426229508196721
24.071067690849304,0.7430441898527005
24.071067690849304,0.7434640522875817
24.071067690849304,0.7438825448613376
24.071067690849304,0.744299674267101
24.071067690849304,0.7447154471544716
24.071067690849304,0.7451298701298701
24.071067690849304,0.7455429497568882
24.071067690849304,0.7459546925566343
24.071067690849304,0.7463651050080775
24.071067690849304,0.7467741935483871
24.82842707633972,0.7471819645732689
24.82842707633972,0.7459807073954984
24.82842707633972,0.7463884430176565
24.82842707633972,0.7467948717948718
24.82842707633972,0.7472
24.82842707633972,0.7476038338658147
24.82842707633972,0.748006379585327
24.82842707633972,0.7484076433121019
24.82842707633972,0.7488076311605724
24.82842707633972,0.7492063492063492
25.313708305358887,0.7496038034865293
25.313708305358887,0.7484177215189873
25.313708305358887,0.7488151658767772
25.313708305358887,0.749211356466877
25.313708305358887,0.7496062992125985
25.313708305358887,0.75
25.313708305358887,0.7488226059654631
25.313708305358887,0.7492163009404389
25.313708305358887,0.7480438184663537
25.313708305358887,0.7484375
25.41421353816986,0.7472698907956318
25.41421353816986,0.7476635514018691
25.41421353816986,0.7480559875583204
25.41421353816986,0.7484472049689441
25.41421353816986,0.7488372093023256
25.41421353816986,0.7476780185758514
25.41421353816986,0.7480680061823802
25.41421353816986,0.7469135802469136
25.41421353816986,0.7473035439137135
25.41421353816986,0.7461538461538462
25.485281229019165,0.7465437788018433
25.485281229019165,0.7469325153374233
25.485281229019165,0.7473200612557427
25.485281229019165,0.7477064220183486
25.485281229019165,0.7480916030534351
25.485281229019165,0.7469512195121951
25.485281229019165,0.745814307458143
25.485281229019165,0.7462006079027356
25.485281229019165,0.7465857359635811
25.485281229019165,0.746969696969697
25.55634891986847,0.7473524962178517
25.55634891986847,0.7477341389728097
25.55634891986847,0.7481146304675717
25.55634891986847,0.7469879518072289
25.55634891986847,0.7473684210526316
25.55634891986847,0.7462462462462462
25.55634891986847,0.7466266866566716
25.55634891986847,0.7455089820359282
25.55634891986847,0.7443946188340808
25.55634891986847,0.744776119402985
25.899494767189026,0.7451564828614009
25.899494767189026,0.7455357142857143
25.899494767189026,0.7459138187221397
25.899494767189026,0.7462908011869436
25.899494767189026,0.7466666666666667
25.899494767189026,0.7470414201183432
25.899494767189026,0.7459379615952733
25.899494767189026,0.7463126843657817
25.899494767189026,0.7466863033873343
25.899494767189026,0.7470588235294118
26.242640614509583,0.7474302496328928
26.242640614509583,0.7478005865102639
26.242640614509583,0.746705710102489
26.242640614509583,0.7470760233918129
26.242640614509583,0.7474452554744525
26.242640614509583,0.7478134110787172
26.242640614509583,0.7467248908296943
26.242640614509583,0.747093023255814
26.242640614509583,0.7474600870827286
26.242640614509583,0.7463768115942029
26.899494767189026,0.7467438494934877
26.899494767189026,0.7471098265895953
26.899494767189026,0.7474747474747475
26.899494767189026,0.7463976945244957
26.899494767189026,0.7453237410071942
26.899494767189026,0.7456896551724138
26.899494767189026,0.7460545193687231
26.899494767189026,0.7464183381088825
26.899494767189026,0.7467811158798283
26.899494767189026,0.7471428571428571
27.485281229019165,0.7475035663338089
27.485281229019165,0.7478632478632479
27.485281229019165,0.748221906116643
27.485281229019165,0.7485795454545454
27.485281229019165,0.7475177304964539
27.485281229019165,0.7478753541076487
27.485281229019165,0.7468175388967468
27.485281229019165,0.7457627118644068
27.485281229019165,0.7461212976022567
27.485281229019165,0.7450704225352113
27.656854152679443,0.7454289732770746
27.656854152679443,0.7457865168539326
27.656854152679443,0.7461430575035063
27.656854152679443,0.7464985994397759
27.656854152679443,0.7468531468531469
27.656854152679443,0.7472067039106145
27.656854152679443,0.7461645746164575
27.656854152679443,0.745125348189415
27.656854152679443,0.7454798331015299
27.656854152679443,0.7458333333333333
28.38477599620819,0.7447988904299584
28.38477599620819,0.7451523545706371
28.38477599620819,0.7455048409405256
28.38477599620819,0.744475138121547
28.38477599620819,0.7448275862068966
28.38477599620819,0.743801652892562
28.38477599620819,0.7441540577716643
28.38477599620819,0.7431318681318682
28.38477599620819,0.7434842249657064
28.38477599620819,0.7424657534246575
32.24264061450958,0.7414500683994528
32.24264061450958,0.7418032786885246
32.24264061450958,0.7421555252387448
32.24264061450958,0.7425068119891008
32.24264061450958,0.7428571428571429
32.24264061450958,0.7432065217391305
32.24264061450958,0.7435549525101763
32.24264061450958,0.7425474254742548
32.24264061450958,0.7415426251691475
32.24264061450958,0.7418918918918919
33.41421353816986,0.7408906882591093
33.41421353816986,0.7412398921832885
33.41421353816986,0.7415881561238223
33.41421353816986,0.7419354838709677
33.41421353816986,0.7422818791946308
33.41421353816986,0.7426273458445041
33.41421353816986,0.7429718875502008
33.41421353816986,0.7433155080213903
33.41421353816986,0.7436582109479306
33.41421353816986,0.7426666666666667
35.0,0.7430093209054593
35.0,0.7420212765957447
35.0,0.7423638778220452
35.0,0.7427055702917772
35.0,0.7417218543046358
35.0,0.7420634920634921
35.0,0.7410832232496698
35.0,0.741424802110818
35.0,0.7404479578392622
35.0,0.7407894736842106
35.899494767189026,0.7398160315374507
35.899494767189026,0.7388451443569554
35.899494767189026,0.7378768020969856
35.899494767189026,0.7382198952879581
35.899494767189026,0.738562091503268
35.899494767189026,0.7389033942558747
35.899494767189026,0.7392438070404173
35.899494767189026,0.7395833333333334
35.899494767189026,0.7399219765929779
35.899494767189026,0.7402597402597403
39.72792184352875,0.7405966277561609
39.72792184352875,0.7409326424870466
39.72792184352875,0.7399741267787839
39.72792184352875,0.7403100775193798
39.72792184352875,0.7406451612903225
39.72792184352875,0.740979381443299
39.72792184352875,0.7413127413127413
39.72792184352875,0.7416452442159382
39.72792184352875,0.7419768934531451
39.72792184352875,0.7423076923076923
40.79898953437805,0.7426376440460948
40.79898953437805,0.7429667519181585
40.79898953437805,0.7420178799489144
40.79898953437805,0.7410714285714286
40.79898953437805,0.7401273885350318
40.79898953437805,0.7404580152671756
40.79898953437805,0.7407878017789072
40.79898953437805,0.7398477157360406
40.79898953437805,0.7401774397972116
40.79898953437805,0.740506329113924
41.14213538169861,0.7408343868520859
41.14213538169861,0.73989898989899
41.14213538169861,0.7402269861286255
41.14213538169861,0.7405541561712846
41.14213538169861,0.740880503144654
41.14213538169861,0.7399497487437185
41.14213538169861,0.740276035131744
41.14213538169861,0.7393483709273183
41.14213538169861,0.7396745932415519
41.14213538169861,0.74
41.97056245803833,0.7403245942571786
41.97056245803833,0.7406483790523691
41.97056245803833,0.7409713574097135
41.97056245803833,0.7412935323383084
41.97056245803833,0.7416149068322981
41.97056245803833,0.7406947890818859
41.97056245803833,0.7410161090458488
41.97056245803833,0.7413366336633663
41.97056245803833,0.7404202719406675
41.97056245803833,0.7407407407407407
43.97056245803833,0.7410604192355117
43.97056245803833,0.7401477832512315
43.97056245803833,0.7404674046740467
43.97056245803833,0.7407862407862408
43.97056245803833,0.7398773006134969
43.97056245803833,0.7401960784313726
43.97056245803833,0.7405140758873929
43.97056245803833,0.7408312958435208
43.97056245803833,0.7411477411477412
43.97056245803833,0.7414634146341463
44.426406145095825,0.7417783191230207
44.426406145095825,0.7408759124087592
44.426406145095825,0.741190765492102
44.426406145095825,0.7402912621359223
44.426406145095825,0.7406060606060606
44.426406145095825,0.7409200968523002
44.426406145095825,0.7412333736396615
44.426406145095825,0.7415458937198067
44.426406145095825,0.7406513872135102
44.426406145095825,0.7409638554216867
47.62741661071777,0.740072202166065
47.62741661071777,0.7403846153846154
47.62741661071777,0.7406962785114045
47.62741661071777,0.7410071942446043
47.62741661071777,0.7413173652694611
47.62741661071777,0.7404306220095693
47.62741661071777,0.7407407407407407
47.62741661071777,0.7410501193317423
47.62741661071777,0.7413587604290822
47.62741661071777,0.7404761904761905
52.97056245803833,0.7395957193816884
52.97056245803833,0.7399049881235155
52.97056245803833,0.7402135231316725
52.97056245803833,0.740521327014218
52.97056245803833,0.7408284023668639
52.97056245803833,0.7411347517730497
52.97056245803833,0.7402597402597403
52.97056245803833,0.7405660377358491
52.97056245803833,0.7408716136631331
52.97056245803833,0.7411764705882353
53.24264061450958,0.7414806110458284
53.24264061450958,0.7406103286384976
53.24264061450958,0.7409144196951934
53.24264061450958,0.7412177985948478
53.24264061450958,0.7415204678362574
53.24264061450958,0.741822429906542
53.24264061450958,0.7421236872812136
53.24264061450958,0.7424242424242424
53.24264061450958,0.7427240977881258
53.24264061450958,0.7430232558139535
54.14213538169861,0.743321718931475
54.14213538169861,0.7424593967517401
54.14213538169861,0.7427578215527231
54.14213538169861,0.7430555555555556
54.14213538169861,0.7433526011560694
54.14213538169861,0.74364896073903
54.14213538169861,0.7427912341407151
54.14213538169861,0.7430875576036866
54.14213538169861,0.7422324510932106
54.14213538169861,0.7425287356321839
54.28427076339722,0.7428243398392652
54.28427076339722,0.7431192660550459
54.28427076339722,0.7434135166093929
54.28427076339722,0.7437070938215103
54.28427076339722,0.744
54.28427076339722,0.7431506849315068
54.28427076339722,0.7434435575826682
54.28427076339722,0.7437357630979499
54.28427076339722,0.7440273037542662
54.28427076339722,0.7443181818181818
55.455843687057495,0.7446083995459705
55.455843687057495,0.7448979591836735
55.455843687057495,0.7451868629671574
55.455843687057495,0.745475113122172
55.455843687057495,0.7457627118644068
55.455843687057495,0.7460496613995485
55.455843687057495,0.7463359639233371
55.455843687057495,0.7454954954954955
55.455843687057495,0.7457817772778402
55.455843687057495,0.7460674157303371
57.65685415267944,0.7463524130190797
57.65685415267944,0.7466367713004485
57.65685415267944,0.7458006718924972
57.65685415267944,0.7460850111856824
57.65685415267944,0.7463687150837989
57.65685415267944,0.7466517857142857
57.65685415267944,0.745819397993311
57.65685415267944,0.7461024498886414
57.65685415267944,0.7452725250278087
57.65685415267944,0.7444444444444445
58.21320307254791,0.7447280799112098
58.21320307254791,0.7450110864745011
58.21320307254791,0.7441860465116279
58.21320307254791,0.7444690265486725
58.21320307254791,0.7436464088397791
58.21320307254791,0.7439293598233996
58.21320307254791,0.743109151047409
58.21320307254791,0.7422907488986784
58.21320307254791,0.7425742574257426
58.21320307254791,0.7428571428571429
58.62741661071777,0.743139407244786
58.62741661071777,0.743421052631579
58.62741661071777,0.7437020810514786
58.62741661071777,0.7428884026258206
58.62741661071777,0.7431693989071039
58.62741661071777,0.7434497816593887
58.62741661071777,0.7437295528898582
58.62741661071777,0.7440087145969498
58.62741661071777,0.7442872687704026
58.62741661071777,0.7445652173913043
59.41421353816986,0.744842562432139
59.41421353816986,0.7440347071583514
59.41421353816986,0.7443120260021668
59.41421353816986,0.7445887445887446
59.41421353816986,0.7448648648648649
59.41421353816986,0.744060475161987
59.41421353816986,0.7443365695792881
59.41421353816986,0.7446120689655172
59.41421353816986,0.7448869752421959
59.41421353816986,0.7451612903225806
60.14213538169861,0.7454350161117078
60.14213538169861,0.7457081545064378
60.14213538169861,0.7459807073954984
60.14213538169861,0.7462526766595289
60.14213538169861,0.7454545454545455
60.14213538169861,0.7457264957264957
60.14213538169861,0.7459978655282817
60.14213538169861,0.746268656716418
60.14213538169861,0.7465388711395101
60.14213538169861,0.7468085106382979
63.426406145095825,0.7460148777895855
63.426406145095825,0.7462845010615711
63.426406145095825,0.7465535524920467
63.426406145095825,0.746822033898305
63.426406145095825,0.7470899470899471
63.426406145095825,0.7473572938689218
63.426406145095825,0.747624076029567
63.426406145095825,0.7468354430379747
63.426406145095825,0.7471022128556375
63.426406145095825,0.7473684210526316
76.62741661071777,0.7476340694006309
76.62741661071777,0.7478991596638656
76.62741661071777,0.7471143756558237
76.62741661071777,0.7473794549266247
76.62741661071777,0.7476439790575916
76.62741661071777,0.7468619246861925
76.62741661071777,0.7471264367816092
76.62741661071777,0.7473903966597077
76.62741661071777,0.7476538060479666
76.62741661071777,0.7479166666666667
79.4558436870575,0.7481789802289281
79.4558436870575,0.7474012474012474
79.4558436870575,0.7476635514018691
79.4558436870575,0.7479253112033195
79.4558436870575,0.7481865284974093
79.4558436870575,0.7484472049689441
79.4558436870575,0.7487073422957601
79.4558436870575,0.7489669421487604
79.4558436870575,0.7492260061919505
79.4558436870575,0.7494845360824742
81.35533845424652,0.7497425334706488
81.35533845424652,0.75
81.35533845424652,0.750256937307297
81.35533845424652,0.7505133470225873
81.35533845424652,0.7497435897435898
81.35533845424652,0.75
81.35533845424652,0.7502558853633572
81.35533845424652,0.7505112474437627
81.35533845424652,0.7507660878447395
81.35533845424652,0.75
83.18376553058624,0.7492354740061162
83.18376553058624,0.7484725050916496
83.18376553058624,0.7477110885045778
83.18376553058624,0.7479674796747967
83.18376553058624,0.7482233502538072
83.18376553058624,0.7484787018255578
83.18376553058624,0.7487335359675785
83.18376553058624,0.7479757085020243
83.18376553058624,0.7482305358948432
83.18376553058624,0.7484848484848485
88.76955199241638,0.7487386478304743
88.76955199241638,0.7479838709677419
88.76955199241638,0.7482376636455186
88.76955199241638,0.7474849094567404
88.76955199241638,0.7477386934673367
88.76955199241638,0.7479919678714859
88.76955199241638,0.7472417251755266
88.76955199241638,0.7474949899799599
88.76955199241638,0.7477477477477478
88.76955199241638,0.748
96.66904675960541,0.7482517482517482
96.66904675960541,0.7485029940119761
96.66904675960541,0.748753738783649
96.66904675960541,0.749003984063745
96.66904675960541,0.7492537313432835
96.66904675960541,0.7495029821073559
96.66904675960541,0.7497517378351539
96.66904675960541,0.7490079365079365
96.66904675960541,0.7492566897918731
96.66904675960541,0.7495049504950495
101.0538227558136,0.7487636003956478
101.0538227558136,0.7490118577075099
101.0538227558136,0.7492596248766041
101.0538227558136,0.7495069033530573
101.0538227558136,0.7487684729064039
101.0538227558136,0.7490157480314961
101.0538227558136,0.7492625368731564
101.0538227558136,0.74950884086444
101.0538227558136,0.7497546614327772
101.0538227558136,0.75
140.0538227558136,0.7502448579823702
140.0538227558136,0.7504892367906066
140.0538227558136,0.750733137829912
140.0538227558136,0.7509765625
140.0538227558136,0.751219512195122
140.0538227558136,0.7514619883040936
140.0538227558136,0.7517039922103214
140.0538227558136,0.7519455252918288
140.0538227558136,0.7521865889212828
140.0538227558136,0.7524271844660194
145.4385987520218,0.7526673132880698
145.4385987520218,0.752906976744186
145.4385987520218,0.7531461761858664
145.4385987520218,0.753384912959381
145.4385987520218,0.7526570048309179
145.4385987520218,0.7519305019305019
145.4385987520218,0.7521697203471552
145.4385987520218,0.7524084778420038
145.4385987520218,0.7516843118383061
145.4385987520218,0.7519230769230769
157.32590091228485,0.7521613832853026
157.32590091228485,0.7523992322456814
157.32590091228485,0.7526366251198466
157.32590091228485,0.7528735632183908
157.32590091228485,0.75311004784689
157.32590091228485,0.7533460803059273
157.32590091228485,0.7535816618911175
157.32590091228485,0.7538167938931297
157.32590091228485,0.7540514775977121
157.32590091228485,0.7542857142857143
200.04163014888763,0.7545195052331113
200.04163014888763,0.7547528517110266
200.04163014888763,0.7549857549857549
200.04163014888763,0.7552182163187856
200.04163014888763,0.7554502369668247
200.04163014888763,0.7547348484848485
200.04163014888763,0.7549668874172185
200.04163014888763,0.7551984877126654
200.04163014888763,0.7554296506137866
200.04163014888763,0.7556603773584906
974.9087229967117,0.7549481621112158
974.9087229967117,0.7551789077212806
974.9087229967117,0.7554092191909689
974.9087229967117,0.7556390977443609
974.9087229967117,0.7549295774647887
974.9087229967117,0.7551594746716698
974.9087229967117,0.7553889409559512
974.9087229967117,0.7556179775280899
974.9087229967117,0.7558465855940131
974.9087229967117,0.7560747663551401

